InternAgent-1.5: A Unified Agentic Framework for Long-Horizon Autonomous Scientific Discovery

We introduce InternAgent-1.5, a unified system designed for end-to-end scientific discovery across computational and empirical domains. The system is built on a structured architecture composed of three coordinated subsystems for generation, verification, and evolution. These subsystems are supported by foundational capabilities for deep research, solution optimization, and long horizon memory. The architecture allows InternAgent-1.5 to operate continuously across extended discovery cycles while maintaining coherent and improving behavior. It also enables the system to coordinate computational modeling and laboratory experimentation within a single unified system. We evaluate InternAgent-1.5 on scientific reasoning benchmarks such as GAIA, HLE, GPQA, and FrontierScience, and the system achieves leading performance that demonstrates strong foundational capabilities. Beyond these benchmarks, we further assess two categories of discovery tasks. In algorithm discovery tasks, InternAgent-1.5 autonomously designs competitive methods for core machine learning problems. In empirical discovery tasks, it executes complete computational or wet lab experiments and produces scientific findings in earth, life, biological, and physical domains. Overall, these results show that InternAgent-1.5 provides a general and scalable framework for autonomous scientific discovery.

==> sections/multiagent_ai_scientist_report.tex <==
% \documentclass{article} % For LaTeX2e
% \usepackage{../iclr2026_conference,times}

% % 你自己需要的宏包（geometry、setspace 就不要了，ICLR 模板已设定好格式）
% \usepackage{hyperref}
% \usepackage{url}
% \usepackage{graphicx}
% \usepackage{booktabs}
% \usepackage{amsmath,amssymb}

% \usepackage{enumitem}

% \setcounter{secnumdepth}{0}


% \title{Research Report on the Latest Progress of Multi-Agent AI Scientists in 2025}
% \author{}

% \begin{document}
% \maketitle
% \newpage
\begin{center}
  % {\LARGE An Example of Full Deep Research Report}\\[4pt]
  {\LARGE Multi-Agent AI Scientists in 2025}
\end{center}
\section*{Introduction}
With the rapid development of Large Language Models (LLMs) and Multi-Agent System (MAS) technologies, 2025 has seen the emergence of a series of ``multi-agent AI scientist'' platforms capable of collaboratively carrying out the entire process of scientific research. This report aims to provide a comprehensive reference for researchers and practitioners by synthesizing the latest definitions, historical background, core methodologies, datasets and evaluation benchmarks, real-world application cases, as well as the challenges faced and directions for future development in the field of multi-agent AI scientists in 2025.

\section*{Overview of Methods / Workflows}
This report is based on a comprehensive analysis of multi-node workflows, drawing mainly on three core sections: (i) background and methods review, (ii) datasets and applications summary, and (iii) analysis of challenges and future directions. Each section compiles key insights from academic papers, industry blogs, white papers, technical reports, and authoritative surveys, preserving original references and data rigorously.

\section*{Findings and Synthesis}

\subsection*{1. Background and Methods}

\subsubsection*{1.1 Definitions}
\begin{itemize}[leftmargin=1.2em]
\item \textbf{Multi-Agent System (MAS)} --- a computerized system composed of multiple interacting agents (software, robots, humans, or hybrids). Core features include autonomy, local views (no global state), and decentralization. Typical research themes encompass agent communication and coordination, distributed problem solving, multi-agent learning, DCOPs, BDI architectures, and LLM-based MAS.
\item \textbf{Multi-Agent ``AI Scientist''} --- a specialized MAS in which agents collaborate to complete the end-to-end scientific research process: hypothesis generation, experimental design, data interpretation, manuscript writing, and peer review. These systems are built upon advances in LLMs: each agent is usually an LLM or LLM+tools, specialized for a specific subtask of the scientific method.
\end{itemize}

\subsubsection*{1.2 Historical Development and Background}

\paragraph{(a) Milestones in Laboratory Automation}
\begin{itemize}[leftmargin=1.2em]
\item \textbf{1875}: First reports of automated scientific equipment, custom-built by scientists to address lab problems.
\item \textbf{Post--WWII}: Commercial vendors began offering increasingly complex automated lab equipment.
\item \textbf{1981--1983}: Dr.\ Masahide Sasaki established the first fully automated laboratory.
\item \textbf{1993}: Dr.\ Rod Markin developed the first clinical laboratory management system and led CTASSC (Clinical Testing Automation Standards Steering Committee).
\item \textbf{2004}: The NIH Roadmap emphasized molecular libraries and imaging technologies, driving large-scale automation in biomedical research.
\item \textbf{Mid-2010s}: Rise of commercial ``on-demand'' remote labs (e.g., Emerald Cloud Lab, Strateos); studies showed that over 90\% of methods in biomedical papers could be accessed through such services.
\item \textbf{Low-cost automation era}: Scripting languages (e.g., AutoIt) and open-source modules (LEGO, 3D printers) lowered the barrier for small labs.
\end{itemize}

\paragraph{(b) Early ``Robot Scientist'' Prototypes}
\begin{itemize}[leftmargin=1.2em]
\item \textbf{Adam (Robot Scientist)} by Ross King et al.\ --- the first system to autonomously discover new knowledge in yeast functional genomics. Capabilities included hypothesis generation, experimental design, robotic execution, results interpretation, and iterative experimentation (domain: \emph{Saccharomyces cerevisiae}).
\item \textbf{Eve} --- a successor system focused on automated drug screening and reproducibility testing in cancer research.
\end{itemize}

\paragraph{(c) Conceptual Basis: MAS}
Traditional MAS research emphasizes communication, coordination, distributed problem solving, multi-agent learning, DCOPs, and BDI-style architectures.

\paragraph{(d) Shift to AI-Driven MAS for Scientific Research}
Advances in LLMs have enabled specialized agents to handle scientific subtasks (literature review, hypothesis generation, coding, data analysis, writing, peer review). Pipelines evolved from single tools to multi-agent workflows orchestrated by a central controller, simulating the iterative cycle of the scientific method. Human intervention is minimized: humans primarily handle wet-lab work and final oversight, while AI agents manage creativity, design, execution, analysis, and writing.

\paragraph{(e) Representative Prototypes and Frameworks before 2025}
\begin{itemize}[leftmargin=1.2em]
\item \textbf{``Lab in the Loop'' (FutureHouse \& Oxford) --- System: Robin}. Agents: Crow \& Falcon (literature analysis; Crow summarizes topics and proposes experimental designs; Falcon writes extended technical reports), Finch (data analysis of raw data such as RNA-seq and flow cytometry), and a Tournament Judge (hypothesis ranking using Bradley--Terry paired comparisons). Closed-loop iterations proceed as Crow/Falcon $\rightarrow$ Finch $\rightarrow$ Judge. In roughly ten weeks, the system completed drug repurposing studies for ten diseases and identified candidate compounds for dry age-related macular degeneration (dry AMD). Humans performed wet-lab experiments and finalized the manuscript.
\item \textbf{Zochi (Intology)} --- a pipeline of retrieval, hypothesis generation, code execution, analysis, writing, and optional automated peer review. Human intervention occurs only ahead of major computation and during final polishing (figures, citations, formatting). Reported outcomes include ACL~2025 acceptance (average reviewer score 4.0), and projects such as CS-ReFT and Tempest/Siege.
\item \textbf{The AI Scientist (Sakana.ai)} --- a four-stage loop: \emph{Idea Generation} (guided by code templates and Semantic Scholar search), \emph{Experimental Iteration} (running and logging code experiments with quantitative/visual outputs), \emph{Paper Write-Up} (LaTeX drafts with auto-citations), and \emph{Automated Peer Review} (LLM-driven near-human feedback). The loop is open-ended (each round is archived and informs the next). Estimated cost is approximately \$15 per paper. Known limitations include lack of precise layout/typography control, occasional implementation bugs, and security concerns when running unsandboxed code.
\end{itemize}

\subsubsection*{1.3 Common Architectural Themes}
\begin{itemize}[leftmargin=1.2em]
\item \textbf{Agent specialization} across subtasks: literature, hypothesis, coding, analysis, writing, and review.
\item \textbf{Workflow orchestration}: centralized coordination following the scientific method's sequence.
\item \textbf{Iterative cycles}: hypothesis $\rightarrow$ experiment $\rightarrow$ analysis $\rightarrow$ refinement.
\item \textbf{Minimal human intervention}: humans focus on wet-lab work and final polishing.
\item \textbf{Automated quality control}: hypothesis ranking (e.g., Bradley--Terry), LLM-based peer review, and meta-analysis.
\end{itemize}

\subsubsection*{1.4 Evolving Standards and Frameworks}
\begin{itemize}[leftmargin=1.2em]
\item Legacy MAS protocols (e.g., KQML, ACL, FIPA) are increasingly complemented or replaced by LLM-driven frameworks (e.g., CAMEL).
\item Safety and ethics considerations include sandboxing, traceability, transparent AI attribution, and biosafety/software-security safeguards.
\end{itemize}

\subsubsection*{1.5 Pioneering Works}
\begin{enumerate}[leftmargin=1.2em]
\item \textbf{Lu et al., ``The AI Scientist: Towards Fully Automated Open-Ended Scientific Discovery''} (arXiv:2408.06292, Sep 2024). First comprehensive LLM-agent framework spanning idea generation, code execution, visualization, manuscript writing, and review loops; estimated cost $<$\$15 per paper; code: \url{https://github.com/SakanaAI/AI-Scientist}.
\item \textbf{Su et al., ``Many Heads Are Better Than One: Improved Scientific Idea Generation by an LLM-Based Multi-Agent System''} (arXiv:2410.09403, May 2025; ACL 2025). Introduces Virtual Scientists (VirSci)---a set of specialized LLMs that generate, evaluate, and optimize research ideas---outperforming single-agent baselines.
\item \textbf{Ghareeb et al., ``Robin: A Multi-Agent System for Automating Scientific Discovery''} (arXiv:2505.13400, May 2025 submission). A closed-loop ``lab-in-the-loop'' MAS integrating literature review, hypothesis generation, experiment design, data analysis, and iterative refinement.
\end{enumerate}

\subsubsection*{1.6 Representative Methods and Model Architectures}
\paragraph{(a) System Goals and Benefits}
These systems address dynamic, dependency-rich research tasks; enable parallel exploration; compress and merge context; and, compared with single-agent baselines, can deliver performance gains on the order of $\sim$90.2\% at the cost of roughly $15\times$ token usage.

\paragraph{(b) Orchestrator--Worker Pattern}
A \emph{Lead (Orchestrator) Agent} analyzes user queries, drafts strategies, persists plans, spawns/monitors subagents, synthesizes outputs, and manages loop termination. \emph{Subagents (Workers)} execute specialized tasks in parallel (e.g., web retrieval, data extraction) using interleaved thinking strategies to optimize queries and return structured results. A dedicated \emph{CitationAgent} can post-process documents to produce precise citations.

\paragraph{(c) Model Backends and Tool Interfaces}
Representative configurations include a powerful model for the lead agent (e.g., Claude Opus~4) and more efficient models for subagents (e.g., Claude Sonnet~4). Tool access is mediated by the Model Context Protocol (MCP) for network search, document retrieval, and workspace APIs. Dynamic multi-step retrieval often replaces static RAG, guided by in-prompt tool-selection heuristics.

\paragraph{(d) Prompt-Engineering Principles}
\begin{enumerate}[leftmargin=1.2em]
\item Simulate agent execution to expose prompt failure modes.
\item Teach the orchestrator to delegate: clarify goals, output schemas, and tool guidance.
\item Scale the number of agents and tool calls with query complexity.
\item Design clean, purpose-built tools.
\item Let agents diagnose and improve other agents' prompts and tool use.
\item Start broad, then progressively focus query strategies.
\item Use extended thinking as an explicit scratchpad.
\item Parallelize tool calls to reduce latency by up to 90\%.
\end{enumerate}

\paragraph{(e) Evaluation Strategies}
Small-sample trials ($\sim$20 queries) assess prompt and tool efficacy; LLM-as-judge scoring covers factuality, citation accuracy, completeness, source quality, and efficiency. Human evaluation supplements these metrics to surface hallucinations and biases. Outcome-centric evaluations focus on persistent state changes.

\paragraph{(f) Production Engineering and Reliability}
Stateful execution, checkpointing and retries; full tracing of agent decisions and tool calls; progressive (``rainbow'') deployment; external storage for plan digests and artifacts; and artifact systems to reduce token costs.

\paragraph{(g) Architectural Challenges and Future Directions}
Synchronizing subagents remains a bottleneck (driving interest in asynchronous coordination). High operational costs encourage focusing on high-value domains. Coupling across subtasks and global-context management also remain open challenges.

\subsection*{2. Datasets, Benchmarks, and Application Cases}

\subsubsection*{2.1 Datasets}
\paragraph{(a) AI Idea Bench 2025 (arXiv:2504.14191)}
A large-scale benchmark for idea generation covering recent venues (ICLR 2025, CVPR 2024, ECCV 2024, NeurIPS 2024, ICML 2024, NAACL 2024, EMNLP 2024, ACL 2024). It aggregates 3{,}495 target AI papers (post--Oct 10, 2023), plus the five most-cited works for each. Tasks include Idea Multiple-Choice Evaluation (IMCQ), Idea-to-Idea (I2I), and Idea-to-Topic (I2T). Representative results are summarized in Table~\ref{tab:aiideabench}.

\begin{table}[h!]
\centering
\caption{Representative AI Idea Bench 2025 results (illustrative extraction).}
\label{tab:aiideabench}
\begin{tabular}{@{}lccc l@{}}
\toprule
Method & I2T & IMCQ (A/B) & Novelty / Feasibility & Notes \\
\midrule
AI-Scientist & 5.0/5.0 & 3.591 / 2.734 & $17.003\times 10^{-3}$ (highest novelty) & --- \\
AI-Researcher & 4.994/4.995 & 2.807 / 2.024 & $9.728\times 10^{-3}$ (overall feasibility) & --- \\
VIRSCI & 4.974/4.983 & 2.937 / 2.123 & strongest protocol alignment & --- \\
SCIPIP & 4.986/--- & 2.437 / --- & --- & --- \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{(b) Open-Source Image Datasets (DatasetAgent; arXiv:2507.08648)}
A multi-agent pipeline where four specialized agents use multimodal LLMs and an image-optimization toolkit to expand or build datasets according to user specifications. Downstream uses include image classification, detection, and segmentation. Specific source datasets (e.g., COCO, ImageNet) are not enumerated here.

\subsubsection*{2.2 Benchmarks and Evaluation Indicators}
\begin{itemize}[leftmargin=1.2em]
\item \textbf{Stanford HAI 2025 AI Index Report}: a general AI benchmark compendium including emerging multi-agent indicators. Highlights include improvements on MMMU (+18.8pp), GPQA (+48.9pp), and SWE-bench (+67.3pp). Responsibility-focused benchmarks covered include HELM Safety, AIR-Bench, and FACTS. The performance gap between open and closed weights narrows from 8\% to 1.7\%. Multi-agent findings note that language-model agents can surpass humans on time-limited programming tasks.
\item \textbf{DatasetAgent (arXiv:2507.08648)}: evaluated via downstream CV tasks (classification, detection, segmentation); the abstract reports methodology without detailed aggregate metrics.
\end{itemize}

\subsubsection*{2.3 Real-World Applications and Case Studies}
\paragraph{(a) Google AI Co-Scientist}
A Gemini 2.0--based coalition of agents (Generation, Reflection, Ranking, Evolution, Proximity, Meta-review) supervised by a \emph{Supervisor} agent. Capabilities include iterative self-debate and tournament-style ranking (Elo-like), automated literature review, hypothesis generation, proposal writing, experimental design, and recursive self-critique. Demonstrations:
\begin{itemize}[leftmargin=1.2em]
\item \textbf{AML drug repurposing}: AI proposed KIRA6; validated \emph{in vitro} across multiple AML cell lines, showing significant tumor-suppression at clinically relevant concentrations.
\item \textbf{Liver fibrosis targets}: identified epigenetic targets with anti-fibrotic activity in human liver organoids (collaboration with Stanford; $p<0.01$).
\item \textbf{Antimicrobial resistance mechanisms}: reproduced cf-PICI host-range expansion mechanisms with timelines consistent with unpublished experimental results (Fleming Initiative \& Imperial College London).
\end{itemize}

\paragraph{(b) Stanford Virtual Lab of AI Scientists}
An AI Principal Investigator agent coordinates subagents spanning immunology, computational biology, and machine learning, along with critic agents. Workflow: a human states a scientific challenge, the AI PI assigns roles, the agents conduct a parallel ``lab meeting'' lasting seconds to minutes and record meeting minutes, and tools such as AlphaFold assist in experimental design. A case study on SARS-CoV-2 vaccine design selected nanobody candidates that were validated for stability, variant binding, and low off-target effects by Chan Zuckerberg Biohub, demonstrating the acceleration provided by autonomous, high-throughput virtual experimentation.

\paragraph{(c) PriM: Principle-Inspired Material Discovery (arXiv:2504.08810)}
A language-reasoning multi-agent system combining domain principles to guide exploration of chemical space via hypothesis generation and round-table MAS discussion. Demonstrated higher discovery rates and improved material properties in a nano-helix materials case compared with baselines. Code/data: \url{https://github.com/amair-lab/PriM}.

\paragraph{(d) SparksMatter: Autonomous Inorganic Materials Discovery (arXiv:2508.02956)}
A GPT-4--series multi-agent framework (\emph{Scientist}, \emph{Planner}, \emph{Assistant}, \emph{Critic}) following the idea$\rightarrow$plan$\rightarrow$experiment$\rightarrow$report pipeline. Integrated tools include the Materials Project API, MatterGen, MatterSim, and CGCNN. Demonstration tasks:
\begin{itemize}[leftmargin=1.2em]
\item \textbf{Green thermoelectrics}: proposed Zintl phase CaMg$_2$Si$_2$ with energy above the convex hull $\leq 0.05\,\mathrm{eV/atom}$; predicted band gap $0.556\,\mathrm{eV}$ and bulk modulus $54.5\,\mathrm{GPa}$, with follow-up validation plans.
\item \textbf{Soft inorganic semiconductors}: identified Hg$_2$MgRb$_2$ (bulk modulus $K=19.94\,\mathrm{GPa}$; band gap $1.52\,\mathrm{eV}$; energy above hull $0.036\,\mathrm{eV/atom}$) including structure and synthesis routes.
\item \textbf{Lead-free perovskite oxides}: selected KNaNb$_2$O$_6$ isotypes ( $E_{\mathrm{hull}} < 0.03\,\mathrm{eV/atom}$; band gap $\approx 2.4\,\mathrm{eV}$; bulk modulus $\approx 98\,\mathrm{GPa}$ ) with ferroelectric potential and validation strategies.
\end{itemize}
Benchmarking indicates superior novelty, depth, and rigor relative to OpenAI o3 / o3-deep-research / o4-mini-deep-research baselines; the authors identify scientific limitations and propose concrete improvements. Code/data: \url{https://github.com/lamm-mit/SparksMatter}.

\section*{Challenges, Limitations, and Future Work}

\subsection*{3.1 Major Challenges and Systemic Risks}
(IONI.ai Compliance Blog, Feb 15, 2025)
\begin{enumerate}[leftmargin=1.2em]
\item \textbf{Agent failures}: errors from a single agent can cascade. Mitigation: data-governance policies, pre-deployment testing, and fault isolation.
\item \textbf{Coordination complexity}: task allocation and messaging protocols are hard, especially with diverse agent roles. Mitigation: layered, sequential, or bidirectional coordination frameworks.
\item \textbf{Unpredictable / emergent behaviors}: decentralized agents may conflict or act unexpectedly. Mitigation: real-time monitoring, conflict-resolution protocols, and human-in-the-loop control.
\item \textbf{Development and deployment challenges}: deep planning is required for multi-agent integration. Best practices: phased rollouts, continuous monitoring, and simulation-based validation.
\item \textbf{Scalability issues}: increasing agent counts and task complexity introduce compute/network bottlenecks. Solutions: dynamic resource allocation, infrastructure optimization, scalable coordination algorithms.
\item \textbf{Security and privacy}: sensitive data traversing multiple agents increases risk. Measures: end-to-end encryption, strict access controls, and periodic security audits.
\item \textbf{Troubleshooting complexity}: emergent behaviors and dependencies complicate debugging. Tools: comprehensive logging, distributed tracing, unified monitoring dashboards.
\item \textbf{Ethics and bias}: data biases can be amplified in hypothesis generation and experimental design. Mitigation: bias audits, fairness-aware algorithms, and diverse training corpora.
\end{enumerate}

\subsection*{3.2 Domain-Specific Limitations in Science}
(Google Research Blog, Feb 19, 2025)
\begin{enumerate}[leftmargin=1.2em]
\item \textbf{Literature coverage}: cross-disciplinary or non-indexed publications may be missed. Remedy: widen retrieval modules to broader scientific corpora.
\item \textbf{Fact-checking}: proposals and hypotheses may contain factual errors. Remedy: integrate external verification tools and authoritative databases.
\item \textbf{Tool interoperability}: reliance on built-in tools limits domain-specific simulations. Remedy: API-driven plugins for scientific software.
\item \textbf{Evaluation misalignment}: Elo-like metrics can diverge from expert judgment. Remedy: hybrid evaluation combining automated scoring with domain-expert feedback.
\item \textbf{Limited expert validation}: early studies involved small expert cohorts and narrow targets. Remedy: larger-scale, cross-disciplinary expert evaluations to enhance generalization.
\end{enumerate}

\subsection*{3.3 Future Work and Research Directions}
\begin{enumerate}[leftmargin=1.2em]
\item \textbf{Modular collaboration architectures}: decompose the scientific pipeline into Generation, Reflection, Ranking, Evolution, Proximity, and Meta-review modules with encapsulation, transparency, and adaptivity; support tight human--AI collaboration.
\item \textbf{Fusion of generative AI and MAS}: integrate LLM components safely, strengthen coordination and distributed decision-making, ensure ethics and traceability, and optimize resource efficiency.
\item \textbf{Cognitive architectures and distributed MAS}: explore edge computing and network heterogeneity to improve robustness; investigate architectures such as Soar and ACT-R for commonsense reasoning and long-horizon goal management.
\item \textbf{External tools and fact verification}: expand cross-disciplinary retrieval; introduce fact-checking engines and authoritative knowledge bases; build plugin interfaces for scientific software.
\item \textbf{Evaluation and expert collaboration}: move beyond Elo-style metrics with hybrid frameworks; organize broader, more diverse expert reviews; implement Trusted Tester programs.
\item \textbf{Governance and community standards}: develop interoperability protocols, ethics and compliance norms, and reproducibility standards for multi-agent scientist systems; clarify legal accountability and funding mechanisms.
\end{enumerate}

\section*{Conclusion}
By 2025, multi-agent AI scientist technologies have made significant progress across definitions and methods, representative systems, datasets and evaluation benchmarks, and real-world applications, while also clarifying key challenges and avenues for future research. Shared characteristics include agent specialization, pipeline-style workflow orchestration, closed-loop iteration, and minimal human intervention. Real-world cases spanning drug repurposing, vaccine design, and materials discovery demonstrate the potential of multi-agent systems to accelerate scientific discovery. Future work should focus on robustness, safety, ethical compliance, and scalable evaluation frameworks to enable sustainable transition from prototypes to large-scale deployment.

\section*{References}
\begin{itemize}[leftmargin=1.2em]
\item Wikipedia: ``Multi-Agent System.''
\item Constantine Goltsev, Apolo.us Blog: ``Lab in the Loop: From Research Tool to Research Leader'' (May 19, 2025).
\item Intology.ai: ``Zochi ACL 2025 Acceptance'' \& technical report.
\item Sakana.ai Whitepaper: ``The AI Scientist: Towards Fully Automated Open-Ended Scientific Discovery'' (arXiv:2408.06292).
\item Anthropic Engineering Blog: ``How we built our multi-agent research system'' (Jun 13, 2025).
\item Model Context Protocol (MCP) documentation: \url{https://modelcontextprotocol.io/introduction}.
\item Anthropic documentation: Extended and interleaved thinking modes.
\item AI Idea Bench 2025 (arXiv:2504.14191).
\item DatasetAgent for open-source image datasets (arXiv:2507.08648).
\item Stanford HAI --- 2025 AI Index Report.
\item Google Research Blog: ``Accelerating scientific breakthroughs with an AI co-scientist'' (Feb 19, 2025).
\item Stanford Medicine News: ``Researchers create `virtual scientists' to solve complex biological problems'' (Jul 29, 2025).
\item PriM: Principle-Inspired Material Discovery (arXiv:2504.08810).
\item SparksMatter: Autonomous Inorganic Materials Discovery (arXiv:2508.02956).
\end{itemize}

\end{document}
